Microphone Array Signal Processing and Deep Learning for Speech Enhancement

Multi-channel acoustic signal processing is a well-established and powerful tool to exploit the spatial diversity between a target signal and non-target or noise sources for signal enhancement. However, the textbook solutions for optimal data-dependent spatial filtering rest on the knowledge of second-order statistical moments of the signals, which have traditionally been difficult to acquire. In this contribution, we compare model-based, purely data-driven, and hybrid approaches to parameter estimation and filtering, where the latter tries to combine the benefits of model-based signal processing and data-driven deep learning to overcome their individual deficiencies. We illustrate the underlying design principles with examples from noise reduction, source separation, and dereverberation.

==> bio/bio.tex <==
% 5. Short 100-word bios for all authors, including email addresses.

Reinhold Haeb-Umbach (haeb@nt.uni-paderborn.de) is a professor of Communications Engineering at Paderborn University, Germany. 
He holds a Dr.-Ing. degree from RWTH Aachen University, and he has more than 30 years of experience in speech research, which he acquired both in an industrial and academic environment. His main research interests are in speech enhancement, acoustic beamforming and source separation, as well as automatic speech recognition and unsupervised learning from speech and audio. 
He coauthored more than 300 scientific publications, and his students have received several best student paper awards. He is a fellow of the International Speech Communication Association (ISCA) and a fellow of the IEEE.

Tomohiro Nakatani (tnak@ieee.org) received B.E., M.E., and Ph.D. degrees from Kyoto University, Kyoto, Japan, in 1989, 1991, and 2002, respectively. He is a Senior Distinguished Researcher at NTT Communication Science Laboratories, NTT Corporation, Japan. Since joining NTT in 1991, he has been investigating audio signal processing technologies for intelligent human-machine interfaces, including dereverberation, denoising, source separation, and robust ASR. He was a member of the IEEE Signal Processing Society (SPS) Audio and Acoustics Technical Committee from 2009 to 2014, and a member of the IEEE SPS Speech and Language Processing Technical Committee from 2016 to 2021. He is a Fellow Member of IEEE. 

Marc Delcroix (marc.delcroix@ieee.org) received his Ph.D.
degree from Hokkaido University, Japan. He is a distinguished
researcher at NTT Communication Science Laboratories, Kyoto
619-0237, Japan. He is a recipient of the 2006 Student Paper
Award from the IEEE Kansai Section, the 2006 Sato Paper
Award from the Acoustical Society of Japan, and the 2015
IEEE Automatic Speech Recognition and Understanding
Workshop Best Paper Award honorable mention. His research
interests include various aspects of speech and audio signal processing, including speech enhancement and robust speech recognition. He is a Senior Member of IEEE. 

Christoph Boeddeker (boeddeker@nt.upb.de) received the bachelor's and master's degrees in electrical engineering from Paderborn University, where he is currently working toward the Ph.D.~degree, under the supervision of Reinhold Haeb-Umbach.
His research interests range from multichannel speech separation, beamforming, and dereverberation to automatic speech recognition on meetings with a focus on combining statistical models and neural networks.
In 2017 and 2022 he pursued a research internship with Microsoft Research, Redmond, USA and MERL, Cambridge, USA, respectively. He is a Member of IEEE. 

Tsubasa Ochiai (tsubasa.ochiai.ah@hco.ntt.co.jp)
received his Ph.D. degree from Doshisha University. He is a
researcher at NTT Communication Science Laboratories,
Kyoto 619-0237, Japan. He is a recipient of the 2014 Student
Presentation Award from the Acoustical Society of Japan
(ASJ), the 2015 Student Paper Award from the IEEE Kansai
Section, the 2020 Awaya Prize Young Researcher Award from
the ASJ, and the 2021 Itakura Prize Innovative Young
Researcher Award from the ASJ. His research interests include
speech enhancement, array signal processing, and robust automatic speech recognition. He is a Member of IEEE.


==> content/beamforming.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{sidebar} 
{\large{Statistically Optimum Beamforming}}
%\doublespacing
\label{sidebar:statistically_optimum_beamforming}

\noindent
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
We consider the signal model of \cref{eq:mtf}, assume a single source ($K=1$) and remove the index $k$ to simplify the notation: $\vect{y}_{t,f} = \vect{h}_f s_{t,f} + \vect{n}_{t,f}$.
Since $\vect{h}_f\cdot s_{t,f} = (\vect{h}_fC)\cdot (s_{t,f}/C)$, where $C\in\mathbb{C}$ is an arbitrary constant, the speech signal can only be recovered up to a multiplicative constant.
That scale ambiguity can be fixed by normalizing the \gls{ATF} $\vect{h}$ to a reference channel (here channel \#1), resulting in the so-called \gls{RTF} $\vect{a}_{f} = \vect{h}_{f}/h_{f,d=1}$, which yields
\begin{align}
	\label{eq:mtf_with_rtf}
	\vect{y}_{t,f} &=  \frac{\vect{h}_{f}}{h_{f,d=1}}\cdot \left(h_{f,d=1}s_{t,f}\right) + \vect{n}_{t,f} =  \vect{a}_{f} x_{t,f,d=1} + \vect{n}_{t,f}.
\end{align}
The goal of beamforming is now to recover the so-called spatial image $x_{t,f,d=1}$ of the target speech signal at a reference microphone, which results in noise reduction, but not in dereverberation\diff{!}{.}

Statistical estimation theory has been employed to derive estimators.
% If the desired signal and the noise are assumed to be normally distributed, the optimal \gls{MMSE} estimator is linear
If the desired signal and the noise are normally distributed, the optimal \gls{MMSE} estimator is linear
\begin{align}
	\label{eq:beamformer_output}
	\hat{x}_{t,f,d=1} = \left(\vect{w}_{f}^{\text{MWF}}\right)^{\HT}\vect{y}_{t,f}
\end{align}
where the so-called \gls{MWF} is the solution of
\begin{align}
	\vect{w}^{\text{MWF}}_{f} &= \argmin_{\vect{w}}\ExpOp\left[|\vect{w}^{\HT}\vect{y}_{t,f} - x_{t,f,d=1}|^2 \right]
 = \argmin_{\vect{w}}\, \hspace{-0.5em}\left.\left\{ \ExpOp\left[|\vect{w}^\HT\vect{x}_{t,f} - x_{t,f,d=1}|^2 \right] + \mu \ExpOp\left[|\vect{w}^\HT \vect{n}_{t,f}|^2\right]\right\}\right|_{\mu=1}\hspace{-0.3em}.
\end{align}
Here, we see that the distortion consists of two terms, the first being the speech distortion and the second the noise term, which we can trade off with the choice of the parameter $\mu$.
The solution to this optimization problem is known as \gls{SDW} \gls{MWF}\cite{gannot2017consolidated}
\begin{align}
	\label{eq:sdw_mwf_solution}
	\vect{w}_{f}^{\text{SDW-MWF}} &= \frac{\left(\scmtrue_{\vect{n},f}\right)^{-1}\vect{a}_f}{\mu + \vect{a}_f^{\HT}\left(\scmtrue_{\vect{n},f}\right)^{-1}\vect{a}_f}
	= \frac{\left(\scmtrue_{\vect{n},f}\right)^{-1}\scmtrue_{\vect{x},f}}{\mu + \tr\left\{\left(\scmtrue_{\vect{n},f}\right)^{-1}\scmtrue_{\vect{x}_f}\right\}} \vect{u}_1
\end{align}
where $\vect{u}_1$ is an all-zero vector with a one at the position of the reference microphone, and $\tr(\cdot)$ is the trace operator.
In these equations, $\scmtrue_{\vect{x},f}= \ExpOp[\vect{x}_{t,f}\vect{x}_{t,f}^\HT]= \vect{a}_f\vect{a_f^\HT}\ExpOp[|x_{t,f,d=1}|^2]$ and $\scmtrue_{\vect{n},f}=\ExpOp[\vect{n}_{t,f}\vect{n}_{t,f}^\HT]$ are the \glspl{SCM} of the speech and the noise part of the microphone signal, respectively.
Setting $\mu=0$ the SDW-MWF identifies with the \gls{MVDR} beamformer:
$\vect{w}_{f}^{\text{MVDR}}= \left.\vect{w}_{f}^{\text{SDW-MWF}}\right|_{\mu=0}$, which optimizes the following constrained minimization $\vect{w}_{f}^{\text{MVDR}} = \argmin_{\vect{w}}\{\vect{w}^\HT\scmtrue_{\vect{n},f}\vect{w}\}$ subject to $\vect{a}_{f}^\HT\vect{w}=1$.
It is important to note that \gls{MWF}, SDW-MWF and other beamformers not discussed here can be implemented as $\vect{w}_{f}^{\text{MVDR}} \cdot C_{f}$, i.e.,  as an \gls{MVDR} beamformer, followed by a single-channel postfilter $C_{f}$.
\end{sidebar}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> response/citefix.tex <==
% This is a bit annoying, but better than manual.
% https://tex.stackexchange.com/questions/378160/how-to-customize-bibtex-numbering-in-a-document

\usepackage{xpatch} % also loads expl3

%%START
\makeatletter
\xpatchcmd{\@bibitem}
  {\item}
  {\item[\@biblabel{\changekey{#1}}]}
  {}{}
\xpatchcmd{\@bibitem}
  {\the\value{\@listctr}}
  {\changekey{#1}}
  {}{}
\makeatother

\ExplSyntaxOn
\cs_new:Npn \changekey #1
 {
  \str_case:nVF {#1} \g_changekey_list_tl { ?? }
 }
\cs_new_protected:Npn \setchangekey #1 #2
 {
  \tl_gput_right:Nn \g_changekey_list_tl { {#1}{#2} }
 }
\tl_new:N \g_changekey_list_tl
\cs_generate_variant:Nn \str_case:nnF { nV }
\ExplSyntaxOff

%Watanabe2020CHiME6,yoshioka2022vararray,meta_smart_glass,Haeb-Umbach_2019

\setchangekey{yoshioka2022vararray}{3}
\setchangekey{Haeb-Umbach_2019}{4}

\setchangekey{Watanabe2020CHiME6}{18}
\setchangekey{cornell23_chime7}{19}

\setchangekey{wang2018multi}{25}
\setchangekey{wang2021multi}{26}

\setchangekey{zmolikova2023masked}{30}
\setchangekey{wisdom2020mom}{31}
\setchangekey{Drude_2019b}{32}
\setchangekey{szegedy2013DNNAdversarialAttack}{32}


\setchangekey{boeddeker2018chime5}{41}
\setchangekey{graetzer2021clarity}{1}
\setchangekey{somasundaram2023projectAria}{2}
\setchangekey{Xiao2016}{49}
\setchangekey{zhang2021adl}{48}
\setchangekey{VINCENT2017535}{33}
\setchangekey{gannot2017consolidated}{9}
\setchangekey{Tzinis_2019}{38}


% https://tex.stackexchange.com/a/18192/148912
\makeatletter
\newcommand{\dummylabel}[2]{%
	\protected@write \@auxout {}{\string \newlabel {#1}{#2}}}
\makeatother

	
\dummylabel{sec:data_denoising}{{\mbox  {III-B}1}{11}}
\dummylabel{sec:model_beamforming}{{\mbox  {III-A}1}{7}}
\dummylabel{sec:model_dereverberation}{{\mbox  {III-A}2}{9}}


\dummylabel{sec:beamforming_case_study}{{\mbox  {IV-E}}{19}}
\dummylabel{sec:joint_model_data_driven_enhancement}{{\mbox  {IV-A}}{15}}
\dummylabel{sec:joint_model_data_driven_parameter}{{\mbox  {IV-B}}{16}}
\dummylabel{sec:modeldeficiencies}{{\mbox  {IV-C}}{18}}
\dummylabel{sec:end-to-end}{{\mbox  {IV-D}}{18}}


\dummylabel{eq:EM:posterior@cref}{{[equation][11][]11}{[1][8][]8}}

==> response/highlight.tex <==
% This code is from Andrew Stacey
% https://tex.stackexchange.com/a/46471/148912
% 
% Examples:
%    \highlight<2>{only on slide 2}
%    \highlight{text to be highlighted}
%    \hlstart text to be highlighted \hlend
% 
% highlighter colour
\makeatletter

%
% Highlighter code
%
\newcommand{\inred}[1]{ {\color{red}  #1}}

\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  save picture id/.code={%
    \edef\pgf@temp{#1}%
    \immediate\write\pgfutil@auxout{%
      \noexpand\savepointas{\pgf@temp}{\pgfpictureid}}%
  }
}

\def\savepointas#1#2{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
}

\tikzdeclarecoordinatesystem{pic}{%
  \@ifundefined{save@pt@#1}{%
    \pgfpointorigin
  }{%
  \pgfsys@getposition{\csname save@pt@#1\endcsname}\save@orig@pic%
  \pgfsys@getposition{\pgfpictureid}\save@this@pic%
  \pgf@process{\pgfpointorigin\save@this@pic}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@process{\pgfpointorigin\save@orig@pic}%
  \advance\pgf@x by -\pgf@xa
  \advance\pgf@y by -\pgf@ya
  }%
}

\newcounter{highlight}
\newcommand{\hlstart}{\tikz[remember picture with id=hlstart\the\value{highlight},baseline=-0.7ex];\hl@start}
\newcommand{\hlend}{\tikz[remember picture with id=hlend\the\value{highlight},baseline=-0.7ex];\hl@end\stepcounter{highlight}}
\newcommand{\fdstart}{\tikz[remember picture with id=hlstart\the\value{highlight},baseline=-0.7ex];\fd@start}
\newcommand{\fdend}{\tikz[remember picture with id=hlend\the\value{highlight},baseline=-0.7ex];\fd@end\stepcounter{highlight}}
\newcommand{\vlstart}{\tikz[remember picture with id=hlstart\the\value{highlight},baseline=-1em];\vl@start}
\newcommand{\vlend}{\tikz[remember picture with id=hlend\the\value{highlight},baseline=0.3ex];\vl@end\stepcounter{highlight}}

\newcommand{\hl@start}[1][]{%
  \hl@draw{highlighter}{#1}{\the\value{highlight}}}

\newcommand{\hl@end}{}

\newcommand{\fd@start}[1][]{%
  \def\fd@args{#1}}

\newcommand{\fd@end}{\def\@tempa{\hl@draw{fader}}\expandafter\@tempa\expandafter{\fd@args}{\the\value{highlight}}\def\fd@args{}}

\newcommand{\vl@start}[1][]{%
  \vl@draw{highlighter}{#1}{\the\value{highlight}}}

\newcommand{\vl@end}{}


\def\hl@sets{%
  \edef\hl@sx{\the\pgf@x}%
  \edef\hl@sy{\the\pgf@y}%
}
\def\hl@sete{%
  \edef\hl@ex{\the\pgf@x}%
  \edef\hl@ey{\the\pgf@y}%
}

\@ifclassloaded{beamer}{

\def\page@node{
  \path (current page.south east)
      ++(-\beamer@rightmargin,\footheight)
  node[
    minimum width=\textwidth,
    minimum height=\textheight,
    anchor=south east
  ] (page) {};
}

}{

  \def\page@node{
    \path (current page.north west)
    ++(\hoffset + 1in + \oddsidemargin + \leftskip,\voffset + 1in + \topmargin + \headheight + \headsep)
    node[
      minimum width=\textwidth - \leftskip - \rightskip,
      minimum height=\textheight,
      anchor=north west
    ] (page) {};
  }

}

\newcommand{\hl@draw}[3]{%
  \begin{tikzpicture}[remember picture,overlay]%
  \page@node
  \tikzset{#2,highlight=#1,every path/.append style={highlight=#1}}%
  \pgfmathsetlengthmacro{\hl@width}{\the\pgflinewidth - 1pt}%
  \coordinate (hlstart) at (pic cs:hlstart#3);
  \coordinate (hlend) at (pic cs:hlend#3);
  \tikz@scan@one@point\hl@sets(pic cs:hlstart#3)
  \tikz@scan@one@point\hl@sete(pic cs:hlend#3)
  \ifdim\hl@sy=\hl@ey\relax
  \draw (hlstart) -- (hlend);
  \else
  \draw (hlstart) -- (hlstart -| page.east);
  \pgfmathsetlengthmacro{\hl@sy}{\hl@sy -\hl@width}%
  \pgfmathsetlengthmacro{\hl@ey}{\hl@ey +\hl@width}%
  \loop\ifdim\hl@sy>\hl@ey\relax
  \draw (0,\hl@sy -| page.west) -- (0,\hl@sy -| page.east);
  \pgfmathsetlengthmacro{\hl@sy}{\hl@sy -\hl@width}%
  \repeat
  \draw (hlend -| page.west) -- (hlend);
  \fi
  \end{tikzpicture}%
}

\newcommand{\vl@draw}[3]{%
  \begin{tikzpicture}[remember picture,overlay]%
  \page@node
  \tikzset{#2,highlight=#1,every path/.append style={highlight=#1}}%
  \pgfmathsetlengthmacro{\hl@width}{\the\pgflinewidth - 1pt}%
  \coordinate (hlstart) at (pic cs:hlstart#3);
  \coordinate (hlend) at (pic cs:hlend#3);
  \tikz@scan@one@point\hl@sets(pic cs:hlstart#3)
  \tikz@scan@one@point\hl@sete(pic cs:hlend#3)
  \ifdim\hl@sx=\hl@ex\relax
  \draw (hlstart) -- (hlend);
  \else
  \draw (hlstart) -- (hlstart |- page.south);
  \pgfmathsetlengthmacro{\hl@sx}{\hl@sx -\hl@width}%
  \pgfmathsetlengthmacro{\hl@ex}{\hl@ex +\hl@width}%
  \loop\ifdim\hl@sx>\hl@ex\relax
  \draw (\hl@sx,0 |- page.north) -- (\hl@sx,0 |- page.south);
  \pgfmathsetlengthmacro{\hl@sx}{\hl@sx -\hl@width}%
  \repeat
  \draw (hlend |- page.north) -- (hlend);
  \fi
  \end{tikzpicture}%
}

\tikzset{%
  highlight/.default=highlighter,
  highlight/.style={
    color=\pgfkeysvalueof{/tikz/#1 colour},
    line width=\pgfkeysvalueof{/tikz/#1 width},
    line cap=\pgfkeysvalueof{/tikz/#1 cap},
    opacity=\pgfkeysvalueof{/tikz/#1 opacity},
  },
  highlighter colour/.initial=yellow,
  highlighter width/.initial=12pt,
  highlighter cap/.initial=butt,
  highlighter opacity/.initial=1,
  fader colour/.initial=gray,
  fader width/.initial=12pt,
  fader cap/.initial=butt,
  fader opacity/.initial=.5,
}



\@ifclassloaded{beamer}{

%% Beamer variants

\setbeamercolor{highlighted text}{bg=yellow}
\setbeamercolor{faded text}{fg=gray}

\newcommand<>{\highlight}[2][]{%
  \only#3{\hlstart[#1]}#2\only#3{\hlend}}

\newcommand<>{\fade}[2][]{%
  \only#3{\fdstart[#1]}#2\only#3{\fdend}}

\newcommand<>{\vhighlight}[2][]{%
  \only#3{\vlstart[#1]}#2\only#3{\vlend}}

}{

\newcommand{\highlight}[2][]{%
\hlstart[#1]#2\hlend}

\newcommand{\fade}[2][]{%
\fdstart[#1]#2\fdend}

\newcommand{\vhighlight}[2][]{%
\vlstart[#1]#2\vlend}

}

\makeatother

